Free Public Transport: More Jobs without Environmental Damage?

We study the effects of a free-fare transport policy implemented by Brazilian localities on employment and greenhouse gas emissions. Using a staggered difference-in-differences approach, we find that fare-free transit increases employment by 3.2% and reduces emissions by 4.1%, indicating that transport policies can decouple economic activity from environmental damage. Our results are driven by workers transitioning from higher-emission to lower-emission sectors instead of being driven by a decline in private transportation use. Cost-benefit analyses suggest that the costly policy only presents net benefits after considering the tax inflows of the increased economic activity and the benefits of reduced carbon emissions.

==> Figures/beneficios_medios_politica.tex <==
\begin{figure}[H]
\begin{center}
\caption{Average direct benefits of the policy, by year}
\label{fig:direct_benefits_policy}
\begin{subfigure}{0.70\linewidth}
\caption{Average benefit from reduction in carbon emissions}
\includegraphics[width=0.95\linewidth]{Files/reducao_media_emissoes.png}
\label{fig:reducao_media_emissoes}
\end{subfigure} \\
\begin{subfigure}{0.70\linewidth}
\caption{Average fiscal externality}
\includegraphics[width=0.95\linewidth]{Files/externalidade_fiscal_media.png}
\label{fig:externalidade_fiscal_media}
\end{subfigure}
\end{center}
\footnotesize{\textit{Notes:} This figure presents the estimates for the two types of benefits of the policy. Figure \ref{fig:reducao_media_emissoes} presents the estimates for the average monetary reduction of carbon emissions as defined in \ref{eq:carbon_benefit} and Figure \ref{fig:externalidade_fiscal_media} presents the estimates for the average fiscal externality as defined in Equation \ref{eq:fiscal_externality}. The values are expressed in BRL millions.}
\end{figure}

==> Figures/custo_beneficio_medio.tex <==
\begin{figure}[H]
\begin{center}
\caption{Average cost and direct benefit of the policy, by year}
\label{fig:average_cost_benefit}
\includegraphics[width=0.65\linewidth]{Files/custo_beneficio_medio.png}
\end{center}
\footnotesize{\textit{Notes:} This figure displays the average cost and direct benefit of the policy. The values are expressed in BRL millions.}
\end{figure}

==> Figures/custo_medio_politica.tex <==
\begin{figure}[H]
\begin{center}
\caption{Average cost of the policy, by year}
\label{fig:average_cost_policy}
\includegraphics[width=0.65\linewidth]{Files/custo_medio_politica.png}
\end{center}
\footnotesize{\textit{Notes:} This figure displays the average cost of the policy across treated municipalities, defined as the product of the average annual individual cost with urban transportation and the average population. The values are expressed in BRL millions.}
\end{figure}

==> Figures/gwp_100_ar5_ghg_vinculos_ativos_calendar.tex <==
\begin{figure}[H]
\begin{center}
\caption{Heterogeneous treatment effects by year for the pre pandemic sample}
\label{fig:gwp_100_ar5_ghg_vinculos_ativos_calendar}
\begin{subfigure}{0.70\linewidth}
\caption{Emissions}
\includegraphics[width=0.95\linewidth]{Files/gwp_100_ar5_ghg_calendar.png}
\label{fig:gwp_100_ar5_ghg_calendar}
\end{subfigure} \\
\begin{subfigure}{0.70\linewidth}
\caption{Employment}
\includegraphics[width=0.95\linewidth]{Files/vinculos_ativos_calendar.png}
\label{fig:vinculos_ativos_calendar}
\end{subfigure}
\end{center}
\footnotesize{\textit{Notes:} This figure presents the estimates of the treatment effects by calendar year from Equation \eqref{eq:treatment_effect_calendar_year}. Figure \ref{fig:gwp_100_ar5_ghg_calendar} presents the dynamic treatment effects on emissions, while Figure \ref{fig:vinculos_ativos_calendar} presents the dynamic treatment effects on employment. The estimation was conducted using the doubly-robust estimator proposed by \cite{callaway2021difference} using a varying base period. Vertical lines represent the 90\% confidence intervals.}
\end{figure}

==> Figures/gwp_100_ar5_ghg_vinculos_ativos_calendar_pandemia.tex <==
\begin{figure}[H]
\begin{center}
\caption{Heterogeneous treatment effects by year}
\label{fig:gwp_100_ar5_ghg_vinculos_ativos_calendar_pandemia}
\begin{subfigure}{0.70\linewidth}
\caption{Emissions}
\includegraphics[width=0.95\linewidth]{Files/gwp_100_ar5_ghg_calendar_pandemia.png}
\label{fig:gwp_100_ar5_ghg_calendar_pandemia}
\end{subfigure} \\
\begin{subfigure}{0.70\linewidth}
\caption{Employment}
\includegraphics[width=0.95\linewidth]{Files/vinculos_ativos_calendar_pandemia.png}
\label{fig:vinculos_ativos_calendar_pandemia}
\end{subfigure}
\end{center}
\footnotesize{\textit{Notes:} This figure presents the estimates of the treatment effects by calendar year from Equation \eqref{eq:treatment_effect_calendar_year}. Figure \ref{fig:gwp_100_ar5_ghg_calendar_pandemia} presents the dynamic treatment effects on emissions, while Figure \ref{fig:vinculos_ativos_calendar_pandemia} presents the dynamic treatment effects on employment. The estimation was conducted using the doubly-robust estimator proposed by \cite{callaway2021difference} using a varying base period. Vertical lines represent the 90\% confidence intervals.}
\end{figure}

==> Figures/gwp_100_ar5_ghg_vinculos_ativos_dynamic.tex <==
\begin{figure}[H]
\begin{center}
\caption{Heterogeneous treatment effects by length of exposure to the treatment for the pre pandemic sample}
\label{fig:gwp_100_ar5_ghg_vinculos_ativos_dynamic}
\begin{subfigure}{0.70\linewidth}
\caption{Emissions}
\includegraphics[width=0.95\linewidth]{Files/gwp_100_ar5_ghg_dynamic.png}
\label{fig:gwp_100_ar5_ghg_dynamic}
\end{subfigure} \\
\begin{subfigure}{0.70\linewidth}
\caption{Employment}
\includegraphics[width=0.95\linewidth]{Files/vinculos_ativos_dynamic.png}
\label{fig:vinculos_ativos_dynamic}
\end{subfigure}
\end{center}
\footnotesize{\textit{Notes:} This figure presents the estimates of the dynamic treatment effects from Equation \eqref{eq:treatment_effect_length_exposure}, both pre and post treatment. Figure \ref{fig:gwp_100_ar5_ghg_dynamic_pandemia} presents the dynamic treatment effects on emissions, while Figure \ref{fig:vinculos_ativos_dynamic_pandemia} presents the dynamic treatment effects on employment. The estimation was conducted using the doubly-robust estimator proposed by \cite{callaway2021difference} using a varying base period and a sample restricted to the pre pandemic years. Vertical lines represent the 90\% confidence intervals.}
\end{figure}

==> Figures/gwp_100_ar5_ghg_vinculos_ativos_dynamic_pandemia.tex <==
\begin{figure}[H]
\begin{center}
\caption{Heterogeneous treatment effects by length of exposure to the treatment}
\label{fig:gwp_100_ar5_ghg_vinculos_ativos_dynamic_pandemia}
\begin{subfigure}{0.70\linewidth}
\caption{Emissions}
\includegraphics[width=0.95\linewidth]{Files/gwp_100_ar5_ghg_dynamic_pandemia.png}
\label{fig:gwp_100_ar5_ghg_dynamic_pandemia}
\end{subfigure} \\
\begin{subfigure}{0.70\linewidth}
\caption{Employment}
\includegraphics[width=0.95\linewidth]{Files/vinculos_ativos_dynamic_pandemia.png}
\label{fig:vinculos_ativos_dynamic_pandemia}\end{subfigure}
\end{center}
\footnotesize{\textit{Notes:} This figure presents the estimates of the dynamic treatment effects from Equation \eqref{eq:treatment_effect_length_exposure}, both pre and post treatment. Figure \ref{fig:gwp_100_ar5_ghg_dynamic_pandemia} presents the dynamic treatment effects on emissions, while Figure \ref{fig:vinculos_ativos_dynamic_pandemia} presents the dynamic treatment effects on employment. The estimation was conducted using the doubly-robust estimator proposed by \cite{callaway2021difference} using a varying base period. Vertical lines represent the 90\% confidence intervals.}
\end{figure}

==> Figures/gwp_100_ar5_ghg_vinculos_ativos_group.tex <==
\begin{figure}[H]
\begin{center}
\caption{Heterogeneous treatment effects by treatment group for the pre pandemic sample}
\label{fig:gwp_100_ar5_ghg_vinculos_ativos_group}
\begin{subfigure}{0.70\linewidth}
\caption{Emissions}
\includegraphics[width=0.95\linewidth]{Files/gwp_100_ar5_ghg_group.png}
\label{fig:gwp_100_ar5_ghg_group}
\end{subfigure} \\
\begin{subfigure}{0.70\linewidth}
\caption{Employment}
\includegraphics[width=0.95\linewidth]{Files/vinculos_ativos_group.png}
\label{fig:vinculos_ativos_group}
\end{subfigure}
\end{center}
\footnotesize{\textit{Notes:} This figure presents the estimates of the group treatment effects from Equation \eqref{eq:treatment_effect_group}. Figure \ref{fig:gwp_100_ar5_ghg_group} presents the group treatment effects on emissions, while Figure \ref{fig:vinculos_ativos_group} presents the dynamic treatment effects on employment. The estimation was conducted using the doubly-robust estimator proposed by \cite{callaway2021difference} using a varying base period and a sample restricted to the pre pandemic years. Horizontal lines represent the 90\% confidence intervals.}
\end{figure}

==> Figures/gwp_100_ar5_ghg_vinculos_ativos_group_pandemia.tex <==
\begin{figure}[H]
\begin{center}
\caption{Heterogeneous treatment effects by treatment group}
\label{fig:gwp_100_ar5_ghg_vinculos_ativos_group_pandemia}
\begin{subfigure}{0.70\linewidth}
\caption{Emissions}
\includegraphics[width=0.95\linewidth]{Files/gwp_100_ar5_ghg_group_pandemia.png}
\label{fig:gwp_100_ar5_ghg_group_pandemia}
\end{subfigure} \\
\begin{subfigure}{0.70\linewidth}
\caption{Employment}
\includegraphics[width=0.95\linewidth]{Files/vinculos_ativos_group_pandemia.png}
\label{fig:vinculos_ativos_group_pandemia}
\end{subfigure}
\end{center}
\footnotesize{\textit{Notes:} This figure presents the estimates of the group treatment effects from Equation \eqref{eq:treatment_effect_group}. Figure \ref{fig:gwp_100_ar5_ghg_group_pandemia} presents the group treatment effects on emissions, while Figure \ref{fig:vinculos_ativos_group_pandemia} presents the dynamic treatment effects on employment. The estimation was conducted using the doubly-robust estimator proposed by \cite{callaway2021difference} using a varying base period. Horizontal lines represent the 90\% confidence intervals.}
\end{figure}

==> Tables/overall_att_estimates_employment_sector_pandemic.tex <==
\begin{table}[H]
\begin{center}
\caption{\label{tab:overall_att_estimates_employment_sector_pandemic}Treatment effects on employment, by sector}
\begin{tabular}{lcccccc}
\toprule
 & Industry & Constr. & Trade & Services & Agriculture & Transp.\\
\midrule
Treatment effect & $0.099^{}$ & $0.247^{*}$ & $-0.015^{}$ & $0.027^{}$ & $-0.049^{**}$ & $-0.056^{}$\\
 & (0.067) & (0.149) & (0.021) & (0.019) & (0.021) & (0.046)\\
\midrule
 Units & 1981 & 976 & 2202 & 2324 & 2161 & 2212\\
Treated units & 40 & 31 & 40 & 40 & 39 & 39\\
Groups & 18 & 14 & 18 & 18 & 18 & 18\\
\bottomrule
\end{tabular}
\end{center}
\footnotesize{\textit{Notes:} This table presents the estimates of the overall treatment effects, defined as in Equation \eqref{eq:overall_treatment_effect}, on the employment of different sectors. The columns indicate the sectors as defined in Table \ref{tab:tab:sector_aggregation}, which are, respectively, industry, construction, trade, services, agriculture, and transportation. The estimation was conducted using the doubly-robust estimator proposed by \cite{callaway2021difference}. Standard errors, clustered at the unit level, are presented in parentheses. Additionally, the table displays the total number of units used in the estimation, along with the number of treated units and treated groups. Significance levels are denoted as follows: $^{***}p<0.01$; $^{**}p<0.05$; $^{*}p<0.1$.}
\end{table}


==> Tables/overall_att_estimates_seeg_ghg_employment.tex <==
\begin{table}[H]
\begin{center}
\caption{\label{tab:overall_att_estimates_seeg_ghg_employment}Treatment effects on emissions and employment}
\centering
\begin{tabular}{lcc}
\toprule
 & GHG emissions & Employment\\
\midrule
Treatment effect & $0.004^{}$ & $0.038^{**}$\\
 & (0.028) & (0.016)\\
\midrule
 Units & 2204 & 2242\\
Treated units & 26 & 26\\
Groups & 17 & 17\\
\bottomrule
\end{tabular}
\end{center}
\footnotesize{\textit{Notes:} This table presents the estimates of the overall treatment effects on emissions and employment, defined as in Equation \eqref{eq:overall_treatment_effect}. The estimation was conducted using the doubly-robust estimator proposed by \cite{callaway2021difference}, using a sample that is restricted to the pre pandemic years. Standard errors, clustered at the unit level, are presented in parentheses. Additionally, the table displays the total number of units used in the estimation, along with the number of treated units and treated groups. Significance levels are denoted as follows: $^{***}p<0.01$; $^{**}p<0.05$; $^{*}p<0.1$.}
\end{table}


==> Tables/overall_att_estimates_seeg_ghg_employment_pandemic.tex <==
\begin{table}[H]
\begin{center}
\caption{\label{tab:overall_att_estimates_seeg_ghg_employment_pandemic}Treatment effects on emissions and employment}
\begin{tabular}{lcc}
\toprule
 & GHG emissions & Employment\\
\midrule
Treatment effect & $-0.043^{*}$ & $0.038^{***}$\\
 & (0.022) & (0.011)\\
\midrule
 Units & 2308 & 2361\\
Treated units & 56 & 41\\
Groups & 20 & 19\\
\bottomrule
\end{tabular}
\end{center}
\footnotesize{\textit{Notes:} This table presents the estimates of the overall treatment effects on emissions and employment, defined as in Equation \eqref{eq:overall_treatment_effect}. The estimation was conducted using the doubly-robust estimator proposed by \cite{callaway2021difference}. Standard errors, clustered at the unit level, are presented in parentheses. Additionally, the table displays the total number of units used in the estimation, along with the number of treated units and treated groups. Significance levels are denoted as follows: $^{***}p<0.01$; $^{**}p<0.05$; $^{*}p<0.1$.}
\end{table}



==> Tables/overall_att_estimates_stock_automobiles_fuel_sales_pandemic.tex <==
\begin{table}[H]
\begin{center}
\caption{\label{tab:overall_att_estimates_stock_automobiles_fuel_sales_pandemic}Treatment effects on stock of automobiles and fuel sales}
\begin{tabular}{lccc}
\toprule
 & Stock of Automobiles & Gasoline sales & Ethanol sales\\
\midrule
Treatment effect & $0.014^{}$ & $0.121^{}$ & $-0.01^{}$\\
 & (0.026) & (0.101) & (0.008)\\
\midrule
 Units & 2,162 & 1,860 & 2,364\\
Treated units & 55 & 52 & 52\\
Groups & 20 & 19 & 15\\
\bottomrule
\end{tabular}
\end{center}
\footnotesize{\textit{Notes:} This table presents the estimates of the overall treatment effects as defined in \eqref{eq:overall_treatment_effect} on the stock of automobiles, gasoline sales and ethanol sales. The estimation was conducted using the doubly-robust estimator proposed by \cite{callaway2021difference}. Standard errors, clustered at the unit level, are presented in parentheses. Additionally, the table displays the total number of units used in the estimation, along with the number of treated units and treated groups. Significance levels are denoted as follows: $^{***}p<0.01$; $^{**}p<0.05$; $^{*}p<0.1$.}
\end{table}

